Variable Markov dynamics as a multi-focal lens to map multi-scale complex networks

From traffic flows on road networks to electrical signals in brain networks, many real-world networks contain modular structures of different sizes and densities. In the networks where modular structures emerge due to coupling between nodes with similar dynamical functions, we can identify them using flow-based community detection methods. However, these methods implicitly assume that communities are dense or clique-like which can shatter sparse communities due to a field-of-view limit inherent in one-step dynamics. Taking multiple steps with shorter or longer Markov time enables us to effectively zoom in or out to capture small or long-range communities. However, zooming out to avoid the field-of-view limit comes at the expense of introducing or increasing a lower resolution limit. Here we relax the constant Markov time constraint and introduce variable Markov dynamics as a multi-focal lens to capture functional communities in networks with a higher range of scales. With variable Markov time, a random walker can keep one-step dynamics in dense areas to avoid the resolution limit and move faster in sparse areas to detect long-range modular structures and prevent the field-of-view limit. We analyze the performance of variable Markov time using the flow-based community detection method called the map equation. We have implemented the map equation with variable Markov time in the search algorithm Infomap without any complexity overhead and tested its performance on synthetic and real-world networks from different domains. Results show that it outperforms the standard map equation in networks with constrained structures and locally sparse regions. In addition, the method estimates the optimal Markov time and avoids parameter tuning.

==> Variable Markov time/SI.tex <==
%\documentclass{article}
%\usepackage[utf8]{inputenc}
%\usepackage{amsmath}
%\usepackage{graphicx}
%\graphicspath{ {./img/} }
%\usepackage{cleveref}
%\usepackage{biblatex}
%\addbibresource{references.bib}
%\usepackage{listings}
%\usepackage{xcolor}
%\definecolor{mygreen}{rgb}{0,0.6,0}
%\definecolor{mygray}{rgb}{0.5,0.5,0.5}
%\definecolor{mymauve}{rgb}{0.58,0,0.82}
%\lstset{ 
%  backgroundcolor=\color{white},
%  basicstyle=\footnotesize,
%  breaklines=true,
%  commentstyle=\color{mygreen},
%  keywordstyle=\color{blue},
%  language=python,
%  numbers=none,
%  stringstyle=\color{mymauve}
%}
%
%\title{Supplementary Information}
%\begin{document}
%\maketitle

\renewcommand\thefigure{S\arabic{figure}}    
\setcounter{figure}{0}   

\section{Supplementary Information}

\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.87\textwidth]{figure1}
  \caption{Field-of-view and resolution limits for constant and variable Markov time. A field-of-view limit is an upper scale on the size of a graph structure where the community detection method will over-partition larger structures. A resolution limit on the other hand is a lower scale on the size of a graph structure where the community detection method will under-partition smaller structures. The Markov time is a global resolution parameter that describes the step length of a random walker and can be increased from the default value of 1 to detect larger structures, but this also raises the resolution limit. The chain is kept together in one module in the space above the blue line, which marks the field-of-view limit in terms of a minimum Markov time needed to not break the chain (a). The cliques are detected below the orange line, which marks resolution limits (b). All three parts -- the two cliques and the chain -- are detected Between these limits (c). With constant Markov time, the chain is only detected below length 7 (d,f,h). With Variable Markov time, the field-of-view limit is pushed further away with increasing clique size (e, g), and disappears when the clique size grows the same as the chain (i).}
  \label{si-fig:fov}
\end{figure}

\clearpage

\subsection*{Interpolation between linear and logarithmic scaling using Tsallis entropy}

The Tsallis entropy for a probability distribution $P = \{p_1,p_2,\dots,p_n\}$ over $n$ categories is defined as
%
\begin{equation}
S_q(P) = \frac{k}{q - 1} \left( 1 - \sum_{i=1}^n p_i^q \right),
\end{equation}
%
where $q$ is a real parameter called entropic index and $k$ is a positive constant, hereafter assumed to be $1$.  In the limit as $q \to 1$ we recover the entropy
%
\begin{equation}
S_1(P) =  -\sum_{i=1}^n p_i \ln p_i
\end{equation}
%
which for a uniform distribution becomes $S_1(n) = \ln n$. To follow the convention used for the map equation to measure entropy in bits, the Tsallis entropy for a uniform distribution $p_i = 1/n$ is 
%
\begin{equation}
S_q(n) = \frac{n^{1-q} - 1}{(1-q)\ln 2}
\end{equation}
%
which gives $S_0(n) = (n - 1)/\ln2$ and $S_1(n) = log_2(n)$. To get an interpolator $f_q(n)$ from $f_{q=0}(n) = n$ to $f_{q=1}(n) = \log_2 n$, we define
%
\begin{equation}
f_q(n) = \frac{n^{1-q} - 1}{(1-q) \ln 2} c_s(q) + c_t(q)
\end{equation}
%
where $c_s(0) = \ln2, c_t(0) = 1$ and $c_s(1) = 1, c_t(1) = 0$.
%
To generalize for any real $q \geq 0$ with a smooth transition for the corrections at $q=1$ we adopt the simplest polynomial interpolator from zero to one on the domain $[0,1]$ with zero derivative at $q=1$, $s(q) = x(2 - x)$, and define the scale correction
%
\begin{equation}
    c_s(q) = \begin{cases} (1 - q(2-q)) \ln 2 + q(2 - q) \quad &\text{if }  0 \leq q < 1 \\
    1 &\text{if } q \geq 1
    \end{cases}
\end{equation}
%
and the translation correction
\begin{equation}
    c_t(q) = \begin{cases} 1 - q (2 - q) \quad &\text{if } 0 \leq q < 1 \\ 
    0 &\text{if } q \geq 1.
    \end{cases}
\end{equation}

\clearpage

\subsection*{Variable Markov time in Infomap}

We have implemented variable Markov time in the community detection algorithm Infomap version~2.6.1~\cite{Edler_The_MapEquation_software_2022}.
To enable this feature, use the command line argument \texttt{--variable-markov-time} and optionally \texttt{--variable-markov-damping d} where $d$ is a real number between 0 and~1.
Using the Infomap Python package, variable Markov time is enabled using the class constructor arguments:
\begin{lstlisting}[language=python]
from infomap import Infomap
im = Infomap(variable_markov_time=True, variable_markov_damping=d)
im.read_file("network.net")
im.run()
\end{lstlisting}



%\end{document}

==> Variable Markov time/latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -cd -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk -cd \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -cd -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -cd -lualatex \"$_[0]\"" );
   }
}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -cd -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk -cd \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -cd -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -cd -lualatex \"$_[0]\"" );
   }
}
